Parameter Identification in a Probabilistic Setting

Parameter identification problems are formulated in a probabilistic language, where the randomness reflects the uncertainty about the knowledge of the true values. This setting allows conceptually easily to incorporate new information, e.g. through a measurement, by connecting it to Bayes's theorem. The unknown quantity is modelled as a (may be high-dimensional) random variable. Such a description has two constituents, the measurable function and the measure. One group of methods is identified as updating the measure, the other group changes the measurable function. We connect both groups with the relatively recent methods of functional approximation of stochastic problems, and introduce especially in combination with the second group of methods a new procedure which does not need any sampling, hence works completely deterministically. It also seems to be the fastest and more reliable when compared with other methods. We show by example that it also works for highly nonlinear non-smooth problems with non-Gaussian measures.

==> diff.tex <==
% RCSID:       $Id: diff.tex,v 1.1 2011/12/23 09:58:35 hgm Exp $
% Author:      $Author: hgm $
% Contact:     wire@tu-bs.de
% =================================
%% texfile{
%%  AUTHOR    = "$Author: hgm $",
%%  VERSION   = "$Revision: 1.1 $",
%%  DATE      = "$Date: 2011/12/23 09:58:35 $",
%%  FILENAME  = "$RCSfile: diff.tex,v $"}
%
% =================================


\subsection{Examples with MCMC updating} \label{SS:diff}
%
Our study will start with a relatively simple system and then progress
to more difficult cases, illustrating the Markov chain Monte Carlo (MCMC)
methods of \refSS{mcmc}.  Let us recall that in that case the posterior
is described by changing the distribution of the underlying RVs.

We start with a simple model of steady state heat transfer \cite{Kucherova10}, 
where the energy balance equation leads to
\begin{equation}   \label{eq:BAL1}
 -\divg (\kappa(x,\omega)\nabla u(x,\omega))=f(x,\omega), 
  \textrm{  a.e. } x\in \C{G} \subset \D{R}^2
\end{equation}
where both the heat conductivity $\kappa$ and the right hand side $f$ may be
considered as random fields over a probability space $\vOmega$.  
Thus \refeq{eq:BAL1} is required to hold almost surely in $\omega$, 
i.e.\ $\D{P}$-almost everywhere.  For the sake of simplicity the conductivity 
$\kappa(x,\omega)$  is taken to be a scalar valued random field, although a conductivity tensor would be a more appropriate choice.  First we will not let
$\kappa$ depend on $u$ and \refeq{eq:BAL1} represents linear model. 
To the balance equation one has to add appropriate Dirichlet and Neumann
boundary conditions, given as a a prescribed temperature
 $u_0=20^\circ \text{C}$ and a heat flux $\nu_x=100 \textrm{ Wm}^{-2}$
 on the left side and zero flux on top and bottom
respectively, as shown in \refig{schema}.
This completes the concrete description of the abstract \refeq{eq:I}, where
here there is no time dependence and thus the time derivative terms vanish.

After spatial discretisation by a standard finite element
method into $120$ elements (see \refig{schema}), the problem is further
discretised with the help of random variables as described in \refS{forward}. Following this the problem reduces to the form 
given by \refeq{eq:I-tens} without the first term as mentioned already.  
The system in \refeq{eq:I-tens} is then solved via the methods given
in \cite{BoyLeBYMadE:2010,NouyACM:2010,Zander10}.

\begin{figure}[h!]
\centering
\includegraphics[width=0.68\textwidth]{./figures/Schema}
\caption{Experimental setup.}
\label{F:schema}
\end{figure}

The conductivity parameter $\kappa(x,\omega)$ is first considered in two 
different scenarios: first as a simple random variable---i.e.\ no dependence
on $x\in \C{G}$---and then as a random field.


\subsubsection{Conductivity as a simple random variable}\label{sec:condrv}
%
We take the thermal conductivity $\kappa$ as independent of the coordinates
$x\in \C{G}$, and for simplicity it is we assume it as an a priori normally
distributed variable $\kappa_f=q_f$ with mean value $\EXP{q_f} = 2
\text{ Wm}^{-1} \text{K}^{-1}$ and
standard deviation $0.3$ Wm$^{-1}$K$^{-1}$.

The measurements will be simulated with a `true' value of
$\kappa_t = 2.5\text{ Wm}^{-1} \text{K}^{-1}$.  They are 
performed in each node of the finite element mesh; and further polluted at
each node by independent centred Gaussian noise 
with a standard deviation of $\sigma_{\varepsilon} = 10^\circ\text{C}$. 

\begin{figure}[h!]
\centering
\includegraphics*[width=0.68\textwidth]{./figures/pdfs.jpg}
\caption{Comparison of prior and posterior pdf and the likelihood function.}
\label{F:pdfcomp1}
\end{figure}
In this particular example the identification of $\kappa$ is done in a fully Bayesian manner (see \refeq{eq:iII}) with the help of a
MCMC procedure with $100000$ samples
as described in \refSS{mcmc}.  In \refig{pdfcomp1} we display the  
shape of the prior, the likelihood function, and the posterior probability
density function (pdf),
and compare it to the truth.  We see that the mean and mode of the posterior
---both are often taken as single point estimates---when compared to the prior
have moved in the direction of the truth; and the variance of the posterior
(signifying the uncertainty about the true value) is less than that of the
prior.  Another frequent single point estimate is the maximum of the likelihood
function---the well known maximum likelihood estimate $L_{\max}(\kappa)$---which
may be seen as also being close to the truth.  One may also observe that
these (and other) point estimates give only an incomplete picture,
as they will not contain information on the residual uncertainty.  
The Bayesian identification procedure on the other hand yields a complete
probability distribution which informs also about the residual uncertainty.

\begin{figure}[h!]
\centering
\includegraphics*[width=0.68\textwidth]{./figures/evolstd.jpg}
\caption{Comparison of the computational times of pure MCMC and PCE based MCMC methods versus the estimate $c_\sigma$.}
\label{F:evolstd}
\end{figure}
The MCMC method performs very well as shown, it is computationally 
very expensive.  It requires the 
calculation of the model response for a large number of samples, each time
solving a FE-system with a different material parameter. 
In order to improve the performance \cite{Marzouk2007,Kucherova10}
we compute a polynomial chaos approximation of the model response by a 
stochastic Galerkin procedure.  Then the 
integration of the posterior distribution may be realised by
sampling the PCE as alluded to at the end of \refS{forward}.
This significantly accelerates the update procedure as shown in 
\refig{evolstd}, where the estimate $c_\sigma:=\sigma (L_{\max}(\kappa))
/\EXP{L_{\max}(\kappa)} )$ is plotted versus computational time
for both the pure and the PCE based MCMC approach.  
Clearly the PCE approximation for the same accuracy of estimate runs 
much quicker than the pure MCMC procedure.

\begin{figure}[h!]
\centering
\includegraphics*[width=0.68\textwidth]{./figures/T-lambda.jpg}
\caption{Polynomial chaos approximation of the model response in one node of computational domain}
\label{F:pcapprox_1}
\end{figure}
The dependence of the PCE on the polynomial order is investigated in
\refig{pcapprox_1} where the accuracy of the temperature approximation in 
one node of the domain is plotted for different polynomial orders. 
Comparing the approximated solution 
with the reference one obtained by MCMC with $100000$ samples
one concludes that only the fifth order approximation can be safely used. 
In this case both responses match. 
Otherwise, for lower values of 
the polynomial order the mean value is estimated 
correctly (the crossing point) but not the higher order moments 
(the lines do not match).
\begin{figure}[h!]
\centering
\includegraphics*[width=0.68\textwidth]{./figures/kld.jpg}
\caption{Kullback-Leibler distance $D(\tilde{\pi}\|\pi)$ from  the posterior obtained by pure MCMC to the PCE reformulated posterior, versus polynomial order}
\label{F:pcapprox_2}
\end{figure}
We try to quantify this discrepancy in \refig{pcapprox_2} in a 
quantitative assessment of the error in the posterior density of the
PCE-based MCMC by computing the Kullback-Leibler divergence (KLD) of
$\tilde{\pi}_{\kappa}$(posterior obtained by PCE/MCMC) from $\pi_{\kappa}$ (posterior obtained by pure MCMC),
\begin{equation}  \label{eq:KLD}
 D(\tilde{\pi}\|\pi) := \int \tilde{\pi}(\kappa)\log 
   \frac{\tilde{\pi}(\kappa)}{\pi(\kappa)}\,\di\kappa.
\end{equation}
This is shown in \refig{pcapprox_2}, where one may observe a rapid rate
of the convergence of the surrogate posterior $\tilde{\pi}_{\kappa}$ to
the true posterior.


\subsubsection{Conductivity as random field}\label{sec:cgrf}
%
The next example is a bit more realistic, by not assuming a priori that
the truth is spatially constant.  
We repeat the previous analysis for the prior $\kappa_f$  being a random
field---again for the sake of simplicity---assumed as Gaussian.
The field $\kappa_f=q_f$ is described by a covariance kernel 
$\exp(-r/l_c)$ with $r$ being the distance and 
$l_c$ a correlation length.
%$l_c=[0.1 \textrm{ }0.04]$ the vector of correlation lengths. 
Furthermore, the mean and standard deviation are chosen in the same manner 
as before (see Section~\ref{sec:condrv}), while the truth is modelled in 
a more realistic way as one realisation of 
the prior field, as shown in \refig{truthfields}. 
All other quantities such as measurement and measurement error stay the 
same as in the previous example.
%
\begin{figure}[h!]
\centering
\begin{tabular}{cc}
\includegraphics*[width=0.48\textwidth]{./figures/2_lambdafield-full.jpg}
&
\includegraphics*[width=0.48\textwidth]{./figures/2_tterr.jpg}
\\
(a) & (b) 
\end{tabular}
\caption{(a) A realisation of the prior random field, 
  (b) Fluctuations of a corresponding temperature field.}
\label{F:truthfields}
\end{figure}


The numerical simulation of the conductivity field is performed by truncating 
the prior KLE (see beginning of this \refS{num-xmpls}) 
to six modes, i.e.\  the random variables $\xi_1 \dots \xi_6$ 
in \refeq{eq:exp-KL} have to be updated.  Similarly as before we use the 
pure MCMC update procedure as well as the PCE based MCMC method. 
The pure MCMC Bayesian update uses $100000$ samples in order to
assimilate the posterior variables, while the PCE approximation is taken 
to be of second order. 
In both cases the updated variables obtain the similar non-Gaussian form as 
shown in \refig{xi_barpdf}~b) and d). In addition, by the comparison 
of the bar-graphs of prior and posterior distributions in \refig{xi_barpdf}~b)
and d) one may see the significant reduction of the prior variance. 
This is clearly visible in  \refig{xi_barpdf}~c) where the probability 
density function of $\xi_5$ is plotted. 
Through the identificaton or assimilation process one obtains from a 
very wide prior distribution a much narrower posterior as expected. 
Also, both methods give very similar results leading to the conclusion that
the error introduced by PCE truncation to second order seems to be 
negligible in this
example.  
%
\begin{figure}[h!]
\centering
\begin{tabular}{cc}
\includegraphics*[width=0.48\textwidth]{./figures/2_smpl_prior_100000.jpg} &
\includegraphics*[width=0.48\textwidth]{./figures/ba.jpg}\\
a) & b)\\
\includegraphics*[width=0.48\textwidth]{./figures/2_pdf_xi5.jpg} &
\includegraphics*[width=0.48\textwidth]{./figures/bo.jpg}\\
c) &d)\\
\end{tabular}
\caption{Distributions of particular random variables: (a) prior, (b) posterior obtained by pure MCMC, (c) pdfs of $\xi_5$, 
(d) posterior obtained using PCE approximation of model response.  In a), b),
and c), the box graphs show for each RV ($\xi_1,\dots,\xi_6$) on the ordinate
the median, the central 25th percentile as a box, the central 75th
percentile, and outliers.}
\label{F:xi_barpdf}
\end{figure}


\subsubsection{Non-linear diffusion} \label{sec:nlindiff}
%
In the isotropic quasi-static diffusion equation given by \refeq{eq:BAL1}, 
we now assume that the conductivity $\kappa$ depends on the 
temperature field $u(x,\omega)$ through
\begin{equation}
\kappa(u,x,\omega) = \kappa_0(x,\omega) + \kappa_1 u(x,\omega) \, ,
\end{equation}
and the previously linear SPDE becomes nonlinear.
Again, just like the prior assumption of a Gaussian conductivity 
before---chosen purely for reasons of simplicity and useful solely because 
the coefficient of variation was very small---is not consistent 
with the requirement by the second law of thermodynamics
that the conductivity be positive, also this linear dependence of
the conductivity can only be seen as a crude approximation, useful only
for a small temperature range.  Its only purpose is to show how the
method works for a simple nonlinear state equation.

\begin{figure}[htpb]
\centering
\begin{tabular}{cc}
\includegraphics*[keepaspectratio,width=5.5cm]{./figures/2_smpl_prior_100000}
&
\includegraphics*[keepaspectratio,width=5.5cm]{./figures/smpl_rwstd=001_100000_tstd=01}
\\
(a) & (b) \\
\includegraphics*[keepaspectratio,width=5.5cm]{./figures/pdf_xi5}
&
\includegraphics*[keepaspectratio,width=5.5cm]{./figures/smpl_rwstd=001_100000_tstd=01_pce}
\\
(c) & (d) 
\end{tabular}
\caption{Distributions of particular random variables: (a) a priori, (b) a posteriori obtained by direct evaluation of the FE model, (c) probability density functions of $\xi_5$, (d) a posteriori obtained using PC approximation of model response.  Box-graphs as in \refig{xi_barpdf}.}
\label{F:nonlpdfs}
\end{figure}

This very simple non-linear constitutive law
is described by two artificial parameters $\kappa_0$ and $\kappa_1$, 
where $\kappa_1 = 0.05\text{ Wm}^{-1}\text{K}^{-2}$ is assumed 
as known and hence is certain,
and $\kappa_0$ is a priori taken as a Gaussian random field
as in the previous Section~\ref{sec:cgrf} with a six term KLE
with mean $ \EXP{\kappa_0}= 2\text{ Wm}^{-1}\text{K}^{-1}$ 
and standard deviation $0.3\text{ Wm}^{-1}\text{K}^{-1}$.  The truth is
taken as one sample of this random field. 
The rest of the experimental set up is taken from the previous tests 
(see the previous Section~\ref{sec:condrv} and \ref{sec:cgrf}).

Similarly as before, the MCMC method in its pure sampling and PCE based form 
is used to calculate the pdfs of the conductivity parameter $\kappa_1$. 
The update procedure consists of assimilation of the six random variables 
$\xi_1,\dots, \xi_6$ of the truncated KLE of the prior field 
$q_f=\kappa_f$  with the help of the temperature measurements in all points 
of the finite element mesh.  Similarly as in the linear case, the box-graphs 
of the prior and posterior random variables in \refig{nonlpdfs}~a) 
and b) show significant reduction of the prior variance and a change 
of the mean, which causes the non-Gaussian form 
of the posterior random variables. 
Furthermore, the comparison of the pure and PCE based MCMC procedure in 
\refig{nonlpdfs}~c) and d) shows that both methods give approximately 
the same results, even though 
the PCE approximation is only of second order.

We see that the MCMC based Bayesian update works also for random fields,
even though the measurement (here the temperature) is not linear in the
quantity to be identified (the conductivity), and also works in case the
state equation is nonlinear.  The inconsistent shape of the prior distribution
(allowing negative conductivities with non-zero probability) is corrected
in all the updates to a form where practically all the probability weight
is in the positive range.  The low order truncated PCE based MCMC performs
almost just as well and is computationally much cheaper---this is 
practically a surrogate model.



%  $Log: diff.tex,v $
%  Revision 1.1  2011/12/23 09:58:35  hgm
%  initial and final (hopefully)
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../12_Sarajevo-main-article"
%%% End: 


